Stable Outcomes and Information in Games: An Empirical Framework

Empirically, many strategic settings are characterized by stable outcomes in which players' decisions are publicly observed, yet no player takes the opportunity to deviate. To analyze such situations in the presence of incomplete information, we build an empirical framework by introducing a novel solution concept that we call Bayes stable equilibrium. Our framework allows the researcher to be agnostic about players' information and the equilibrium selection rule. The Bayes stable equilibrium identified set collapses to the complete information pure strategy Nash equilibrium identified set under strong assumptions on players' information. Furthermore, all else equal, it is weakly tighter than the Bayes correlated equilibrium identified set. We also propose computationally tractable approaches for estimation and inference. In an application, we study the strategic entry decisions of McDonald's and Burger King in the US. Our results highlight the identifying power of informational assumptions and show that the Bayes stable equilibrium identified set can be substantially tighter than the Bayes correlated equilibrium identified set. In a counterfactual experiment, we examine the impact of increasing access to healthy food on the market structures in Mississippi food deserts.

==> Version 5 final/Tables/marginal_effects.tex <==
\begin{tabular}{l*{3}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{In}&\multicolumn{1}{c}{In}&\multicolumn{1}{c}{In}\\
\midrule
Own-brand outlets present in nearby markets&      -0.067&      -0.076&      -0.096\\
                    &     (0.002)&     (0.002)&     (0.002)\\
\addlinespace
Long distance to HQ (> 1.6K km)&      -0.083&      -0.083&      -0.010\\
                    &     (0.003)&     (0.003)&     (0.003)\\
\addlinespace
Many eating/drinking places (>7)&            &       0.203&       0.203\\
                    &            &     (0.002)&     (0.002)\\
\addlinespace
High income per capita (>25K dollars)&            &      -0.038&      -0.037\\
                    &            &     (0.002)&     (0.002)\\
\addlinespace
Low access to healthy food&            &       0.039&       0.041\\
                    &            &     (0.004)&     (0.004)\\
\addlinespace
McDonald's          &            &            &       0.109\\
                    &            &            &     (0.002)\\
\midrule
State Dummies       &         Yes&         Yes&         Yes\\
N                   &     107,042&     107,042&     107,042\\
\bottomrule
\end{tabular}


==> Version 5 final/Tables/summary_statistics.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccccc}}
\toprule
                    &\multicolumn{5}{c}{}                                            \\
                    &        Mean&     Std dev&         Min&         Max&           N\\
\midrule
\textbf{\emph{Decision variables}}&            &            &            &            &            \\
MD Entry            &       0.196&       0.397&        0.00&        1.00&       54940\\
BK Entry            &       0.106&       0.307&        0.00&        1.00&       54940\\
\textbf{\emph{Firm-specific variables}}&            &            &            &            &            \\
MD outlets present in nearby markets&       0.720&       0.449&        0.00&        1.00&       54940\\
BK outlets present in nearby markets&       0.483&       0.500&        0.00&        1.00&       54940\\
Long distance to MD HQ (>1.6K km)&       0.285&       0.451&        0.00&        1.00&       54940\\
Long distance to BK HQ (>1.6K km)&       0.712&       0.453&        0.00&        1.00&       54940\\
\textbf{\emph{Market environment variables}}&            &            &            &            &            \\
Many eating/drinking places (>7 stores)&       0.465&       0.499&        0.00&        1.00&       54940\\
High income per capita (>25K dollars)&       0.502&       0.500&        0.00&        1.00&       54940\\
Low access to healthy food&       0.856&       0.351&        0.00&        1.00&       54940\\
Food desert         &       0.334&       0.472&        0.00&        1.00&       54940\\
\bottomrule
\end{tabular}
}

